KGEx: Explaining Knowledge Graph Embeddings via Subgraph Sampling and Knowledge Distillation

Despite being the go-to choice for link prediction on knowledge graphs, research on interpretability of knowledge graph embeddings (KGE) has been relatively unexplored. We present KGEx, a novel post-hoc method that explains individual link predictions by drawing inspiration from surrogate models research. Given a target triple to predict, KGEx trains surrogate KGE models that we use to identify important training triples. To gauge the impact of a training triple, we sample random portions of the target triple neighborhood and we train multiple surrogate KGE models on each of them. To ensure faithfulness, each surrogate is trained by distilling knowledge from the original KGE model. We then assess how well surrogates predict the target triple being explained, the intuition being that those leading to faithful predictions have been trained on impactful neighborhood samples. Under this assumption, we then harvest triples that appear frequently across impactful neighborhoods. We conduct extensive experiments on two publicly available datasets, to demonstrate that KGEx is capable of providing explanations faithful to the black-box model.

==> proposal.tex <==
\section{FocusE}\label{sec:method}

We present FocusE, an add-on layer for knowledge graph embedding architectures designed for link prediction with numeric-enriched triples.
FocusE takes into account numeric literals associated to each link. Regardless of their semantics, we operate under the assumption that numeric values intensify or mitigate the probability of existence of a link.
For example, given numeric values $w$ in the $[0-1]$ range, we assume that high values identify triples with higher chances of being true, low scores single out weak or unlikely relations, and $w=0$ triples are considered negative samples. 

FocusE consists in a plug-in layer that fits between the scoring and loss layers of a conventional KGE method and it is designed to be used during training (Figure~\ref{fig:arch}).
Unlike traditional architectures, before feeding the scoring layer to a loss function, we modulate its output based on numeric values associated to triples, to obtain ``focused'' scores. 
We leverage numeric values associated to triples so that during training the model focuses on triples with higher numeric values. 
We want our model to learn from training triples with high numeric values, and at the same time use edge numeric values to maximise the margin between scores assigned to true triples and those assigned to their corruptions. This increases the loss of the model and helps it focus on triples with higher values.
Our contribution is described below in detail.


Let $t=(s,p,o)$ be a positive triple and $w>0$ its numeric-value. We define a corruption of $t$ as $t^-=(s,p,o')$ or $t^-=(s',p,o)$. where $s', o'$ are respectively subject or object corruptions.

Let $f(t)$ be the scoring function of a KGE model. In the case of TransE~\cite{bordes2013translating} this is:

\begin{equation}
f(t) = -||\mathbf{e}_{s} + \mathbf{r}_{p} - \mathbf{e}_{o}||_n
\end{equation}

where $\mathbf{e}_{s}$, $\mathbf{r}_{p}$ and $\mathbf{e}_{o}$ are the embeddings of the subject $s$, predicate $p$, and object $o$.

We use a softplus non-linearity $\sigma$ to make sure the scores returned by $f(t)$ are greater or equal to zero, without introducing excessive distortion: %

\begin{equation}
g(t) = \sigma(f(t))= \ln{(1+e^{f(t)})} \geq 0
\end{equation}


To take into account the effect of numeric values associated to triples, we define a modulating factor $\alpha \in \mathbb{R}$ which is responsible to strike a balance between the influence of the structure of the graph and the impact of the numeric values associated to each triple:

\begin{equation}
\alpha =
\begin{cases}
 \beta + (1-w)(1-\beta) & \mbox{if \,} t \\
 \beta + w(1-\beta) & \mbox{if \,} t^-
\end{cases}
\label{eq:alpha}
\end{equation}

where $\beta \in [0,1]$ is the \textit{structural influence}, an hyperparameter that modulates the influence of graph topology, and $w \in \mathbb{R}$ is the numeric value associated to the \textit{positive} triple $t$. 
$\beta$ is used to re-weigh the triple value $w$. If $\beta=0$ the original numeric values $w$ are used. If $\beta=1$, numeric values $w$ are ignored and the model is equivalent to a conventional KGE architecture.
Note that positive and negative triples are assigned different $\alpha$ equations.
This is done to lower the margin between the scores for triples and their respective corruptions when the triple numeric value is high. 

Finally, the FocusE layer $h(t)$ is defined as:

\begin{equation}
h(t) = \alpha \, g(t)
\label{eq:ht}
\end{equation}

Putting all together, the FocusE layer $h(t)$ is then used in the loss function\footnote{Note that the FocusE layer described in Eq.\ref{eq:ht} is compatible with other losses used in KGE literature (e.g. pairwise, negative log-likelihood, etc.)} $L$. 
This is a modified, more numerically stable version of the negative log-likelihood of normalized softmax scores proposed in \cite{kadlec2017knowledge}:

\begin{equation}
L = - \sum_{t^+,t^-} log \frac{e^{h(t^+)}}{e^{h(t^+)} + e^{h(t^-)}} \label{eq:loss}
\end{equation}

As seen in \eqref{eq:loss}, the modulation between structural influence and numeric values increases the margin between high and low-valued triples. Hence the model learns to focus on triples with higher numeric attributes. 

During training, we decay the structural influence $\beta$ from 1 to 0. This is controlled by the hyperparameter $\lambda$ (decay). Initially the model gives equal importance to all training triples. When $\beta$ decays to zero (linearly, over $\lambda$ epochs), the model exclusively relies on numeric attributes ($w$).
Section~\ref{sec:decay} shows empirical evidence of the effectiveness of $\lambda$.




